Mitigating Oversmoothing Through Reverse Process of GNNs for Heterophilic Graphs

Graph Neural Network (GNN) resembles the diffusion process, leading to the over-smoothing of learned representations when stacking many layers. Hence, the reverse process of message passing can produce the distinguishable node representations by inverting the forward message propagation. The distinguishable representations can help us to better classify neighboring nodes with different labels, such as in heterophilic graphs. In this work, we apply the design principle of the reverse process to the three variants of the GNNs. Through the experiments on heterophilic graph data, where adjacent nodes need to have different representations for successful classification, we show that the reverse process significantly improves the prediction performance in many cases. Additional analysis reveals that the reverse mechanism can mitigate the over-smoothing over hundreds of layers. Our code is available at https://github.com/ml-postech/reverse-gnn.

==> fig/homo_main_table_without_std.tex <==
\begin{table}[t!]
    \centering
    \resizebox{.99\linewidth}{!}{
    \begin{tabular}{cccccc} 
         \toprule & Cora & CiteSeer & PubMed & Computers & Photo \\ 
         \midrule
         MLP* & \tabnumwithoutstd{76.96}{0.95} & \tabnumwithoutstd{76.58}{0.88} & \tabnumwithoutstd{85.94}{0.22} & \tabnumwithoutstd{82.85}{0.38} & \tabnumwithoutstd{84.72}{0.34} \\
         vanilla-GCN* & \tabnumwithoutstd{87.14}{1.01} & \tabnumwithoutstd{79.86}{0.67} & \tabnumwithoutstd{86.74}{0.27} & \tabnumwithoutstd{83.32}{0.33} & \tabnumwithoutstd{88.26}{0.73} \\
         vanilla-GAT* & \tabnumwithoutstd{88.03}{0.79} & \besttabnumwithoutstd{80.52}{0.71} & \tabnumwithoutstd{87.04}{0.24} & \tabnumwithoutstd{83.32}{0.39} & \tabnumwithoutstd{90.94}{0.68} \\
         APPNP* & \tabnumwithoutstd{88.14}{0.73} & \underline{\tabnumwithoutstd{80.47}{0.74}} & \tabnumwithoutstd{88.12}{0.31} & \tabnumwithoutstd{85.32}{0.37} & \tabnumwithoutstd{88.51}{0.31} \\
         ChevNet* & \tabnumwithoutstd{86.67}{0.82} & \tabnumwithoutstd{79.11}{0.75} & \tabnumwithoutstd{87.95}{0.28} & \tabnumwithoutstd{87.54}{0.43} & \tabnumwithoutstd{93.77}{0.32} \\
         GPR-GNN* & \besttabnumwithoutstd{88.57}{0.69} & \tabnumwithoutstd{80.12}{0.83} & \tabnumwithoutstd{88.46}{0.33} & \tabnumwithoutstd{86.85}{0.25} & \tabnumwithoutstd{93.85}{0.28} \\
         BernNet* & \underline{\tabnumwithoutstd{88.52}{0.95}} & \tabnumwithoutstd{80.09}{0.79} & \tabnumwithoutstd{88.48}{0.41} & \tabnumwithoutstd{87.64}{0.44} & \tabnumwithoutstd{93.63}{0.35} \\
         \midrule
         GRAND& \tabnumwithoutstd{85.53}{0.64} & \tabnumwithoutstd{74.95}{1.37} & \tabnumwithoutstd{88.81}{0.69} & \tabnumwithoutstd{90.28}{0.47} & \tabnumwithoutstd{94.01}{0.73}\\ 
         GRAND+\ours{}& \tabnumwithoutstd{85.73}{1.39} & \tabnumwithoutstd{75.78}{1.48} & \tabnumwithoutstd{89.03}{0.61} & \tabnumwithoutstd{89.51}{0.78}  & \tabnumwithoutstd{94.48}{0.61} \\ 
         $\Delta$& $+0.20\;(\uparrow)$ & $+0.83\;(\uparrow)$ & $+0.22\;(\uparrow)$ & $-0.77\;(\downarrow)$ & $+0.47\;(\uparrow)$ \\ 
         \midrule
         GAT& \tabnumwithoutstd{87.67}{0.84} & \tabnumwithoutstd{77.36}{1.59} & \tabnumwithoutstd{89.66}{0.60} & \besttabnumwithoutstd{92.15}{0.30} & \besttabnumwithoutstd{95.86}{0.58}\\  
         GAT+\ours{}& \tabnumwithoutstd{87.93}{1.60}  & \tabnumwithoutstd{77.06}{1.60} & \underline{\tabnumwithoutstd{89.94}{0.61}} &\tabnumwithoutstd{91.03}{0.62} &\tabnumwithoutstd{95.44}{0.71} \\  
         & $(64/32)$ & $(32/128)$ & $(8/8)$ & $(16/8)$ & $(32/8)$\\
         $\Delta$& $+0.26(\uparrow)$ & $-0.30(\downarrow)$ & $+0.28(\uparrow)$ & $-1.12(\downarrow)$ & $-0.42(\downarrow)$\\   
         \midrule
         GCN& \tabnumwithoutstd{88.00}{1.42} & \tabnumwithoutstd{77.15}{1.44} & \tabnumwithoutstd{89.37}{0.52} & \underline{\tabnumwithoutstd{91.87}{0.57}} & \tabnumwithoutstd{95.35}{0.47}\\ 
         GCN+\ours{}& \tabnumwithoutstd{87.63}{1.40}  & \tabnumwithoutstd{77.33}{1.65} & \besttabnumwithoutstd{89.96}{0.55} & \tabnumwithoutstd{90.92}{0.52} & \underline{\tabnumwithoutstd{95.50}{0.63}}\\ 
         & $(32/512)$ & $(8/32)$ & $(32/32)$ & $(32/64)$ & $(32/128)$\\
         $\Delta$& $-0.37(\downarrow)$ & $+0.18(\uparrow)$ & $+0.59(\uparrow)$ & $-0.95(\downarrow)$ & $+0.15(\uparrow)$\\  
         \bottomrule
    \end{tabular}
    }
    \caption{Test accuracy and standard deviation on \textit{homophilic} datasets. $\Delta$ indicates the difference with and without \ours. We also report the number of forward and reverse steps below the performance of GCN$+$\ours{} and GAT$+$\ours{}. The best and the second-best are bolded and underlined, respectively.}
    \label{tab:homo_main}
\end{table}

==> fig/intro_minesweeper.tex <==
\begin{figure}[t!]
    \centering
    % \begin{subfigure}{0.48\columnwidth}
    %     \includegraphics[width=\linewidth]{fig/sampled[46,23]_label.png}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.48\columnwidth}
    %     \includegraphics[width=\linewidth]{fig/sampled[46,23]_rep.png}
    % \end{subfigure}

    \includegraphics[width=\linewidth]{fig/minesweeper-illustration.pdf}
    
    \caption{Example of the Minesweeper dataset. On the left, two mines are located on a grid-structured graph with a signal of eight. After diffusion, the signal is propagated to the adjacent nodes. In Minesweeper, we observe the graph on the right and need to find the original location of the mines. If one can reverse the diffusion, the reversion represents the presence of mines.}
    \label{fig:minesweeper}
\end{figure}

==> fig/main_table_backup.tex <==
\begin{table*}
    \centering
    \begin{tabular}{ccccc} 
         \hline & Squirrel-filtered & Chameleon-filtered & roman-empire & amazon-ratings \\
         \hline 
         SAGE & \tabnum{36.09}{1.99} & \tabnum{37.77}{4.14} & \tabnum{85.74}{0.67} & \boldsymbol{\tabnum{53.63}{0.39}}\\
         GAT-sep & \tabnum{35.46}{3.10} & \tabnum{39.26}{2.50} & \boldsymbol{\tabnum{88.75}{0.41}} & \tabnum{52.70}{0.62} \\
         GT & \tabnum{36.30}{1.98} & \tabnum{38.87}{3.66} & \tabnum{86.51}{0.73} & \tabnum{51.17}{0.66} \\
         GT-sep & \tabnum{36.66}{1.63} & \tabnum{40.31}{3.01} & \underline{\tabnum{87.32}{0.39}} & \tabnum{52.18}{0.80} \\
         \hline 
         H2GCN & \tabnum{35.10}{1.15} & \tabnum{26.75}{3.64} & \tabnum{60.11}{0.52} & \tabnum{36.47}{0.23} \\ 
         CPGNN & \tabnum{30.04}{2.03} & \tabnum{33.00}{3.15} & \tabnum{63.96}{0.62} & \tabnum{39.79}{0.77} \\ 
         GPR-GNN & \tabnum{38.95}{1.99} & \tabnum{39.93}{3.30} & \tabnum{64.85}{0.27} & \tabnum{44.88}{0.34} \\
         FSGNN & \tabnum{35.92}{1.32} & \tabnum{40.61}{2.97} & \tabnum{79.92}{0.56} & \tabnum{52.74}{0.83} \\
         GloGNN & \tabnum{35.11}{1.24} & \tabnum{25.90}{3.58} & \tabnum{59.63}{0.69} & \tabnum{36.89}{0.14} \\ 
         FAGCN & \underline{\tabnum{41.08}{2.27}} & \tabnum{41.90}{2.72} & \tabnum{65.22}{0.56} & \tabnum{44.12}{0.30} \\
         GBK-GNN & \tabnum{35.51}{1.65} & \tabnum{39.61}{2.60} & \tabnum{74.57}{0.47} & \tabnum{45.98}{0.71} \\
         JacobiConv & \tabnum{29.71}{1.66} & \tabnum{39.00}{4.20} & \tabnum{71.14}{0.42} & \tabnum{43.55}{0.48} \\
         LRGNN* & \tabnum{39.51}{2.12} & \tabnum{41.24}{2.95} & \tabnum{40.88}{1.84} & \tabnum{42.23}{4.85} \\
         \hline
         GRAND& \tabnum{35.94}{1.64} &  \tabnum{37.71}{4.48} & \tabnum{75.19}{0.56} & \tabnum{49.34}{0.72} \\
         GRAND+\ours{}& \tabnum{40.75}{2.44} &  \tabnum{42.14}{3.62} & \tabnum{77.53}{0.62} & \tabnum{48.30}{0.60} \\ 
         $\Delta$& $+4.81\;(\uparrow)$ & $+4.43\;(\uparrow)$ & $+2.34\;(\uparrow)$ & $-1.04\;(\downarrow)$ \\  
         \hline
         GCN & \tabnum{39.47}{1.47} & \tabnum{40.89}{4.12} & \tabnum{73.69}{0.74} & \tabnum{48.70}{0.63} \\
         % \hline resGCN& $45.8\;(16)$ & $47.94\;(16)$ & $78.5\;(2)$ & $49.52\;(4)$ \\
         % \hline GCN+\ours{}& $47.12\;(64-4)$  & $50.52\;(64-2)$ & $79.49\;(64-1)$ & $51.35\;(64-8)$ \\
         GCN+\ours{}& \boldsymbol{\tabnum{44.73}{2.66}} & \boldsymbol{\tabnum{47.23}{3.76}} & \tabnum{86.76}{0.48} & \underline{\tabnum{52.96}{0.52}} \\
         & $(226/236)$ & $(154/310)$ & $(179/40)$ & $(26/1)$ \\
         $\Delta$& $+5.26\;(\uparrow)$ & $+6.34\;(\uparrow)$ & $+13.07\;(\uparrow)$ & $+4.26\;(\uparrow)$ \\  
         \hline
         GAT & \tabnum{35.62}{2.06} & \tabnum{39.21}{3.08} & \tabnum{80.87}{0.30} & \tabnum{49.09}{0.63} \\
         GAT+\ours{}& \tabnum{40.20}{1.80}  & \underline{\tabnum{44.05}{3.95}} & \tabnum{85.70}{0.72} & \tabnum{52.53}{0.71} \\ 
         & $(48/14)$ & $(206/148)$ & $(57/5)$ & $(21/6)$\\
         $\Delta$& $+4.58\;(\uparrow)$ & $+4.84\;(\uparrow)$ & $+4.83\;(\uparrow)$ & $+3.44\;(\uparrow)$ \\  
         \hline
    \end{tabular}
    \caption{Test accuracy and standard deviation on \textit{heterophilic} graph \red{with first priority}}
    \label{tab:my_label}
\end{table*}

\begin{table}
    \centering
    \resizebox{.99\columnwidth}{!}{
    \begin{tabular}{cccc} 
         \hline & minesweeper & tolokers & questions \\ 
         \hline 
         SAGE & \tabnum{93.51}{0.57} & \tabnum{82.43}{0.44} & \tabnum{76.44}{0.62} \\
         GAT-sep & \tabnum{93.91}{0.35} & \tabnum{83.78}{0.43} & \tabnum{76.79}{0.71} \\
         GT & \tabnum{91.85}{0.76} & \tabnum{83.23}{0.64} & \tabnum{77.95}{0.68} \\
         GT-sep & \tabnum{92.29}{0.47} & \tabnum{82.52}{0.92} & \underline{\tabnum{78.05}{0.93}} \\
         \hline 
         H2GCN & \tabnum{89.71}{0.31} & \tabnum{73.35}{1.01} & \tabnum{63.59}{1.46} \\
         CPGNN & \tabnum{52.03}{5.46} & \tabnum{73.36}{1.01} & \tabnum{65.96}{1.95} \\
         GPR-GNN & \tabnum{86.24}{0.61} & \tabnum{72.94}{0.97} & \tabnum{55.48}{0.91} \\
         FSGNN & \tabnum{90.08}{0.70} & \tabnum{82.76}{0.61} & \boldsymbol{\tabnum{78.86}{0.92}} \\
         GloGNN & \tabnum{51.08}{1.23} & \tabnum{73.39}{1.17} & \tabnum{65.74}{1.19} \\
         FAGCN & \tabnum{88.17}{0.73} & \tabnum{77.75}{1.05} & \tabnum{77.24}{1.26} \\
         GBK-GNN & \tabnum{90.85}{0.58} & \tabnum{81.01}{0.67} & \tabnum{74.47}{0.86} \\
         JacobiConv & \tabnum{89.66}{0.40} & \tabnum{68.66}{0.65} & \tabnum{73.88}{1.16}\\
         LRGNN* & \tabnum{52.66}{6.40} & \tabnum{74.24}{1.37} & \tabnum{66.41}{1.75} \\
         \hline
         GRAND& \tabnum{90.41}{0.78} & \tabnum{78.38}{1.91} & \tabnum{76.22}{1.06}  \\ 
         GRAND+\ours{}& \tabnum{91.42}{0.78} & \tabnum{80.44}{1.64} & \tabnum{76.41}{1.04} \\
         $\Delta$& $+1.01\;(\uparrow)$ & $+2.06\;(\uparrow)$ & $+0.19\;(\uparrow)$\\
         \hline
         GCN & \tabnum{89.75}{0.52} & \tabnum{83.64}{0.67} & \tabnum{76.09}{1.27} \\
         % \hline resGCN& $91.86\;(8)$ & $83.68\;(8)$ & $76.33\;(16)$\\ 
         %\hline GCN+\ours{}& $91.7\;(2-8)$ & $85.02\;(64-4)$ & $76.48\;(64-8)$\\ 
         GCN+\ours{}& \underline{\tabnum{93.98}{0.40}} & \boldsymbol{\tabnum{86.05}{0.68}} & \tabnum{77.78}{1.26} \\ 
         & $(4/86)$ & $(37/116)$ & $(74/68)$ \\
         $\Delta$& $+4.23\;(\uparrow)$ & $+2.41\;(\uparrow)$ & $+1.69\;(\uparrow)$ \\   
         \hline
         GAT & \tabnum{92.01}{0.68} & \tabnum{83.70}{0.47} & \tabnum{77.43}{1.20} \\
         GAT+\ours{}& \boldsymbol{\tabnum{94.11}{0.46}} & \underline{\tabnum{84.83}{0.42}} & \tabnum{76.69}{1.05}\\  
         & $(42/4)$ & $(11/1)$ & $(46/2)$\\
         $\Delta$& $+2.10\;(\uparrow)$ & $+1.13\;(\uparrow)$ & $-0.74\;(\downarrow)$ \\  
         \hline
    \end{tabular}
    }
    \caption{Test ROC AUC and standard deviation on \textit{heterophilic} graph}
    \label{tab:my_label}
\end{table}
